Generating Novel Scene Compositions from Single Images and Videos

Given a large dataset for training, generative adversarial networks (GANs) can achieve remarkable performance for the image synthesis task. However, training GANs in extremely low data regimes remains a challenge, as overfitting often occurs, leading to memorization or training divergence. In this work, we introduce SIV-GAN, an unconditional generative model that can generate new scene compositions from a single training image or a single video clip. We propose a two-branch discriminator architecture, with content and layout branches designed to judge internal content and scene layout realism separately from each other. This discriminator design enables synthesis of visually plausible, novel compositions of a scene, with varying content and layout, while preserving the context of the original sample. Compared to previous single image GANs, our model generates more diverse, higher quality images, while not being restricted to a single image setting. We further introduce a new challenging task of learning from a few frames of a single video. In this training setup the training images are highly similar to each other, which makes it difficult for prior GAN models to achieve a synthesis of both high quality and diversity.

==> figures/bank_sin_im.tex <==
\begin{figure*}[h!]
	\begin{centering}
		\setlength{\tabcolsep}{0.0em}
		\renewcommand{\arraystretch}{0}
		\par\end{centering}
	\begin{centering}
		\vspace{-1.5em}
		%\hfill{}%
		\begin{tabular}{c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}
			
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/single_image_ref_frame_res1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/single_image_gen_4_res1}  &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/single_image_gen_9_res1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/single_image_gen_3_res1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/single_image_gen_0_res1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/single_image_gen_1_res1}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloons_frame_res} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloons_res8} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloons_res1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloons_res4} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloons_res9} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloons_res10}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/garden_frame_res} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/garden_rescr10} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/garden_rescr1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/garden_rescr3} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/garden_rescr9} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/garden_rescr17} \tabularnewline  \hline \hline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/13/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/13/6} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/13/8} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/13/11} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/13/32} &
%			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/13/15_!}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/15/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/15/30} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/15/28_1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/15/20} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/15/32} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/15/13}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/17/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/17/84} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/17/82} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/17/79} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/17/75} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/17/101s}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/19/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/19/62} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/19/4_1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/19/11} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/19/16} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/19/0}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/20/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/20/0} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/20/0_1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/20/1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/20/18_1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/20/5}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/21/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/21/2} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/21/4_2} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/21/15} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/21/23} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/21/14}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/23/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/23/0} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/23/6} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/23/14} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/23/31} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/23/67}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/27/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/27/1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/27/5_1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/27/10} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/27/69} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/27/87}
			\tabularnewline 
			
		
			
			
			%\includegraphics[width=0.32\linewidth]{figures/teaser/two_images_ref}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_1}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_2}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_3}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_4}
			
		\end{tabular}\hfill{}
		\par\end{centering}
	
	\caption{\label{fig:bank_image} Here I put images as candidates for Single Image visuals.}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[h!]
	\begin{centering}
		\setlength{\tabcolsep}{0.0em}
		\renewcommand{\arraystretch}{0}
		\par\end{centering}
	\begin{centering}
		\vspace{-1.5em}
		%\hfill{}%
		\begin{tabular}{c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}
					
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/30/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/30/2} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/30/3} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/30/24} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/30/15} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/30/69}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/38/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/38/0} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/38/0_1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/38/0_2} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/38/3} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/38/20}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/40/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/40/4} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/40/4_1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/40/5} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/40/9} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/40/34}
			\tabularnewline 
			
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/42/ref} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/42/11} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/42/1} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/42/7} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/42/15} &
			\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/42/37}
			\tabularnewline 
			
					\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/50/ref} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/50/1} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/50/13} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/50/14} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/50/15} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/50/19}
		\tabularnewline
		
			
		
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/landscape_person/ref} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/landscape_person/1} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/landscape_person/3} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/landscape_person/5} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/landscape_person/7} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/landscape_person/37}
		\tabularnewline
		
			
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/mountains/ref} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/mountains/0} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/mountains/10} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/mountains/1} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/mountains/2} &
		\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/bank_sin_im/mountains/3}
		\tabularnewline 
			
			%\includegraphics[width=0.32\linewidth]{figures/teaser/two_images_ref}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_1}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_2}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_3}
			%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_4}
			
		\end{tabular}\hfill{}
		\par\end{centering}
	
	\caption{\label{fig:bank_image} Here I put images as candidates for Single Image visuals.}
	\vspace{-1em}
\end{figure*}

==> figures/high_resolution.tex <==
\begin{figure}[t]
	\begin{centering}
		\setlength{\tabcolsep}{0.0em}
		\renewcommand{\arraystretch}{0}
		\par\end{centering}
	\begin{centering}
	%\hfill{}%
	\begin{tabular}{@{\hskip 0.01in}c@{\hskip 0.00in}c}
			

\includegraphics[width=0.16\linewidth, height=0.09\linewidth]{supplementary/figures/higher_res/ref1_frame.jpg} 
\includegraphics[width=0.16\linewidth, height=0.09\linewidth]{supplementary/figures/higher_res/small2.jpg} 
\includegraphics[width=0.16\linewidth, height=0.09\linewidth]{supplementary/figures/higher_res/small3.jpg} 
\includegraphics[width=0.16\linewidth, height=0.09\linewidth]{supplementary/figures/higher_res/small4.jpg} 
\includegraphics[width=0.16\linewidth, height=0.09\linewidth]{supplementary/figures/higher_res/small5.jpg} 
\includegraphics[width=0.16\linewidth, height=0.09\linewidth]{supplementary/figures/higher_res/small1.jpg} 

\tabularnewline 

\includegraphics[width=0.326\linewidth, height=0.18\linewidth]{supplementary/figures/higher_res/Picture2.jpg} 
\includegraphics[width=0.326\linewidth, height=0.18\linewidth]{supplementary/figures/higher_res/Picture4.jpg} 
\includegraphics[width=0.326\linewidth, height=0.18\linewidth]{supplementary/figures/higher_res/Picture6.jpg} 
\tabularnewline  
			
		\end{tabular}\hfill{}
		\par\end{centering}
	\vspace{-0.9em}
	\caption{Generation results from a single image of SIV-GAN trained for different image shapes of 320x192 and 896x512. Our model maintains the quality of synthesis and the ability to vary content and layout of scenes at different image scales, showing good scalability to high resolutions. \vadim{Will try to find replacement for some examples}}
	\label{fig:high_resolution}
\vspace{-2em}
\end{figure}



==> figures/manipulation.tex <==
\begin{figure*}[t]
	\begin{centering}
		\setlength{\tabcolsep}{0.0em}
		\renewcommand{\arraystretch}{0}
		\par\end{centering}
	\begin{centering}
		%\hfill{}%
		\begin{tabular}{c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}}
			
			Single image \& mask & \multicolumn{4}{c}{Image manipulation results using inpainting \cite{dong2022incremental} and object blending \cite{zhang2020deep} methods}
			\tabularnewline 
			
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{supplementary/figures/higher_res/ref1_frame_mask} & 	
			
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{figures/manipulation/0} &
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{figures/manipulation/1} &
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{figures/manipulation/2} &
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{figures/manipulation/4} 
			\tabularnewline 
			
			Training image & \multicolumn{4}{c}{SIV-GAN generation results}
			\tabularnewline 
			
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{supplementary/figures/higher_res/ref1_frame}
			& 
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{supplementary/figures/higher_res/Picture2} &
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{supplementary/figures/higher_res/Picture4} &
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{supplementary/figures/higher_res/Picture6} &
			\includegraphics[width=0.19\linewidth, height=0.11\linewidth]{supplementary/figures/higher_res/Picture5} 
			
		\end{tabular}
		\par\end{centering}
	\vspace{-1.3ex}
	\caption{Comparison of SIV-GAN synthesis to image manipulation methods in the Single Image setting. The ability of SIV-GAN to remove objects from scenes can be performed by image inpaiting \cite{dong2022incremental}, while moving or duplicating objects can be done with an object blending method \cite{zhang2020deep} applied at random locations. Nonetheless, unlike SIV-GAN these methods require object annotations, which can be restrictive in practice. Moreover, image manipulation methods achieve significantly lower diversity, and sometimes suffer from inpainting distortions and unrealistic objects at new locations.}
	\label{fig:manipulation}
	\vspace{-2ex}
\end{figure*}



==> figures/qual_comparison.tex <==
\begin{figure}[t]
\begin{centering}
\setlength{\tabcolsep}{0.0em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
\vspace{-1em}
\hfill{}%
	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c}
			\centering
		Label map & Ground truth & Pix2pixHD & SPADE & CC-FPSE & OASIS\vspace{0.01cm} \tabularnewline
		
%				\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips19_1} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our_1} \tabularnewline
		
				
		
		
		
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/label0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/image0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/pix2pix_0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/spade0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/nips0022} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/our0022} \tabularnewline
		
		
			\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/label1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/image1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/pix2pix_1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/spade1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/nips1879} & {\footnotesize{}}
		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/our1879} \tabularnewline
		
%	
%			\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/label1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/image1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/pix2pix_1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/spade1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/nips1534} & {\footnotesize{}}
%		\includegraphics[width=0.16\textwidth, height=0.08\textheight]{figures/qual_comp/our1534} \tabularnewline
		
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/label_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/image_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/spade_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/nips19_4} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.14\textwidth]{figures/qual_comp/our_4} \tabularnewline
%		

		
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0196} \tabularnewline
		
				
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips19_2} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our_2} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips19_3} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our_3} \tabularnewline
		
%			\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1913} \tabularnewline


	
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1548} \tabularnewline
		
	
		
	
		
	
		
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0058} \tabularnewline
		
	

			\end{tabular}
\hfill{}
\par\end{centering}
\vspace{-0.5em}
\caption{\label{fig:qual_comp} Qualitative comparison of OASIS with other methods on ADE20K. Trained with only adversarial supervision, our model generates images with better perceptual quality and structure.}
\vspace{-1em}
\end{figure}




%\begin{figure}[t]
%\begin{centering}
%\setlength{\tabcolsep}{0.0em}
%\renewcommand{\arraystretch}{0}
%\par\end{centering}
%\begin{centering}
%\vspace{-1em}
%\hfill{}%
%	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
%			\centering
%		Label map & Real image & SPADE \cite{park2019semantic} & CC-FPSE \cite{liu2019learning} & Our model\vspace{0.05cm} \tabularnewline
%
%
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0022} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0022} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0058} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0058} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips0196} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our0196} \tabularnewline
%
%
%			\end{tabular}
%\hfill{}
%\par\end{centering}
%\caption{\label{fig:qual_comp} Qualitative comparison with other methods. Trained without the perceptual loss, our model generates images with better textures, perceptual quality and the color distribution closer to real images. }
%\vspace{-0.5em}
%\end{figure}
%
%
%
%
%
%\begin{figure}[t]
%\begin{centering}
%\setlength{\tabcolsep}{0.0em}
%\renewcommand{\arraystretch}{0}
%\par\end{centering}
%\begin{centering}
%\vspace{-1em}
%\hfill{}%
%	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
%			\centering
%		Label map & Real image & SPADE \cite{park2019semantic} & CC-FPSE \cite{liu2019learning} & Our model\vspace{0.05cm} \tabularnewline
%
%
%
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1534} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1534} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1548} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1548} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1879} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1879} \tabularnewline
%
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/label1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/image1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/spade1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/nips1913} & {\footnotesize{}}
%		\includegraphics[width=0.195\textwidth, height=0.08\textheight]{figures/qual_comp/our1913} \tabularnewline
%
%			\end{tabular}
%\hfill{}
%\par\end{centering}
%\caption{\label{fig:qual_comp} Qualitative comparison with other methods. Trained without the perceptual loss, our model generates images with better textures, perceptual quality and the color distribution closer to real images. }
%\vspace{-0.5em}
%\end{figure}
%
%
%


==> figures/qual_results_2images.tex <==
\begin{figure}[h!]
\begin{centering}
\setlength{\tabcolsep}{0.1em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
\vspace{-1em}
\hfill{}%
\begin{tabular}{c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}


\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat}\tabularnewline

\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat} & {\footnotesize{}}
\includegraphics[width=0.25\linewidth]{figures/funny_cat}\tabularnewline


\end{tabular}\hfill{}
\par\end{centering}
\vspace{-0.5em}
\caption{\label{fig:qual_2image} Some images from 2 image training
 }
\vspace{0em}
\end{figure}

==> figures/teaser.tex <==
\begin{figure*}[h]
\begin{centering}
\setlength{\tabcolsep}{0.1em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
%\vspace{-1.0em}
\hfill{}%
\begin{tabular}{@{\hskip -0.03in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}
	
Training video and samples generated from \emph{a single video} \tabularnewline
\includegraphics[width=0.4845\linewidth]{figures/teaser/car/ref} ~
\includegraphics[width=0.4845\linewidth]{figures/teaser/park/ref} \tabularnewline
%\hspace{0.01em}
\includegraphics[width=0.158\linewidth, height=0.08\textheight]{figures/teaser/car/car_3} 
\includegraphics[width=0.158\linewidth, height=0.08\textheight]{figures/teaser/car/car_1}
\includegraphics[width=0.158\linewidth, height=0.08\textheight]{figures/teaser/car/car_2}  ~
%\includegraphics[width=0.16\linewidth]{figures/teaser/single_video_gen_4} 
%\includegraphics[width=0.16\linewidth]{figures/teaser/single_video_gen_6} 
\includegraphics[width=0.158\linewidth, height=0.08\textheight]{figures/teaser/park/1}
\includegraphics[width=0.158\linewidth, height=0.08\textheight]{figures/teaser/park/32}
\includegraphics[width=0.158\linewidth, height=0.08\textheight]{figures/teaser/park/25}
%\includegraphics[width=0.16\linewidth]{figures/teaser/park1201}
 \tabularnewline  \tabularnewline 
Training image and samples generated from \emph{a single image} \tabularnewline


\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloon/balloons_frame_res}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloon/12}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloon/91}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloon/15}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloon/14}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/balloon/balloons13}


\tabularnewline

%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/teaser/rock/single_image_ref_frame_res1}
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/teaser/rock/0} 
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/teaser/rock/28_1}
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/teaser/rock/30}
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/teaser/rock/32} 
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/teaser/rock/43} 
%\tabularnewline 

\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/fish/ref_frame}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/fish/36}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/fish/8}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/fish/11}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/fish/47}
\includegraphics[width=0.16\linewidth, height=0.08\textheight]{figures/teaser/fish/12}

\tabularnewline

\includegraphics[width=0.325\linewidth, height=0.16\textheight]{figures/teaser/fish/reslarge_wave11}
\includegraphics[width=0.325\linewidth, height=0.16\textheight]{figures/teaser/fish/reslarge_wave8}
\includegraphics[width=0.325\linewidth, height=0.16\textheight]{figures/teaser/fish/reslarge_wave12}



%
%\tabularnewline ~\includegraphics[width=0.326\linewidth]{figures/teaser/fish/reslarge_wave6}
%\includegraphics[width=0.326\linewidth]{figures/teaser/fish/reslarge_wave10}
%\includegraphics[width=0.326\linewidth]{figures/teaser/fish/reslarge_wave7}




%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/bank_sin_im/mountains/ref} 
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/bank_sin_im/mountains/0} 
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/bank_sin_im/mountains/10} 
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/bank_sin_im/mountains/1} 
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/bank_sin_im/mountains/2} 
%\includegraphics[width=0.16\linewidth, height=0.065\textheight]{figures/bank_sin_im/mountains/3}

%~\includegraphics[width=0.16\linewidth, %#height=0.065\textheight]{figures/teaser/garden/garden_frame_res}
%\includegraphics[width=0.16\linewidth, %height=0.065\textheight]{figures/teaser/garden/5_1}
%\includegraphics[width=0.16\linewidth, %height=0.065\textheight]{figures/teaser/garden/garden_rescr1}
%\includegraphics[width=0.16\linewidth, %height=0.065\textheight]{figures/teaser/garden/garden_rescr17}
%\includegraphics[width=0.16\linewidth, %height=0.065\textheight]{figures/teaser/garden/garden_rescr9}
%\includegraphics[width=0.16\linewidth, %height=0.065\textheight]{figures/teaser/garden/87}


%\includegraphics[width=0.32\linewidth]{figures/teaser/two_images_ref}
%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_1}
%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_2}
%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_3}
%\includegraphics[width=0.16\linewidth, height=0.126\linewidth]{figures/teaser/two_images_4}
%\vspace{-1em}
\end{tabular}\hfill{}
\par\end{centering}
\caption{\label{fig:teaser} Images generated by SIV-GAN. Our model successfully operates in extremely low data regimes, generating new scene compositions with varying content and layout from a single video (first two rows) or a single image (last three rows). For example, from the single training video with a car on the road, SIV-GAN generates images without a car or with two cars; and for the single surfing image, it can synthesize layouts with a different position and configuration of waves varying the number of surfers in the scene. SIV-GAN is able to maintain the quality and diversity of scene compositions while operating at different image resolutions, e.g., 192$\times$320 (fourth row) and 512$\times$896 (last row). (Original training samples are shown in grey or red frames.) 
%the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene. change positions and configuration of waves in the see.   
%\caption{\label{fig:teaser} Images generated at different resolutions by SIV-GAN. Our model successfully operates in different extremely low-data regimes, including learning from a single video (first two rows) or a single image (last three rows), generating new scene compositions with varying content and layout. 
%For example, from the single training video with a car on the road, SIV-GAN generates images without a car or with two cars; and for the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene.  
%(Original samples are shown in grey or red frames.) \anna{caption should mention more strongly compositions of new scenes, and point out to high resolution images}
%One-Shot GAN images generated from a single video or a single image. Our model successfully operates in different one-shot settings, including learning from a single video (first two rows) or a single image (last three rows), generating new scene compositions with varying content and layout. 
%For example, from the single training video with a car on the road, One-Shot GAN generates images without a car or with two cars; for the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene.  
%(Original samples are shown in grey or red frames.)
}
%\vspace{-1em}
\end{figure*}

%- For Fig. 1, the caption should provide some additional explanation of the results. For the video, it is discussed in Section 4.3, but since the figure is at the beginning, it is better to give the reviewer directly the text that explains the quality of the results. You might move the figure also to page 2, if the caption gets longer.

==> figures/teaser_onecolumn_image.tex <==
\newcommand\myfigure{ %\begin{figure}[h]
\begin{centering}
\setlength{\tabcolsep}{0.1em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
%\vspace{-1.0em}
\hfill{}%
\begin{tabular}{@{\hskip -0.03in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}


Training image and samples generated from \emph{a single image} \tabularnewline


\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/balloon/balloons_frame_res}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/balloon/12}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/balloon/91} \tabularnewline
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/balloon/15}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/balloon/14}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/balloon/balloons13}


\tabularnewline


\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/fish/ref_frame}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/fish/47}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/fish/11} \tabularnewline
%\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/fish/36}
%\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/fish/12}
%\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/fish/8}

\includegraphics[width=0.485\linewidth, height=0.12\textheight]{figures/teaser/fish/reslarge_wave11}
\includegraphics[width=0.485\linewidth, height=0.12\textheight]{figures/teaser/fish/reslarge_wave12}
 \tabularnewline  \tabularnewline
%\includegraphics[width=0.485\linewidth, height=0.16\textheight]{figures/teaser/fish/reslarge_wave8}
%\tabularnewline


%\vspace{-1em}
\end{tabular}\hfill{}
\par\end{centering}
%\caption{\label{fig:teaser}  shown in grey or red frames.) 
%the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene. change positions and configuration of waves in the see.   
%\caption{\label{fig:teaser} Images generated at different resolutions by SIV-GAN. Our model successfully operates in different extremely low-data regimes, including learning from a single video (first two rows) or a single image (last three rows), generating new scene compositions with varying content and layout. 
%For example, from the single training video with a car on the road, SIV-GAN generates images without a car or with two cars; and for the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene.  
%(Original samples are shown in grey or red frames.) \anna{caption should mention more strongly compositions of new scenes, and point out to high resolution images}
%One-Shot GAN images generated from a single video or a single image. Our model successfully operates in different one-shot settings, including learning from a single video (first two rows) or a single image (last three rows), generating new scene compositions with varying content and layout. 
%For example, from the single training video with a car on the road, One-Shot GAN generates images without a car or with two cars; for the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene.  
%(Original samples are shown in grey or red frames.)
%}
%\vspace{-1em}
}
%\end{figure}

%- For Fig. 1, the caption should provide some additional explanation of the results. For the video, it is discussed in Section 4.3, but since the figure is at the beginning, it is better to give the reviewer directly the text that explains the quality of the results. You might move the figure also to page 2, if the caption gets longer.

==> figures/teaser_onecolumn_video.tex <==
\begin{figure}[h]
\begin{centering}
\setlength{\tabcolsep}{0.1em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
%\vspace{-1.0em}
\hfill{}%
\begin{tabular}{@{\hskip -0.03in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}


Training video and samples generated from \emph{a single video} \tabularnewline 
\includegraphics[width=0.98\linewidth]{figures/teaser/car/ref} \tabularnewline 
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/car/car_3} 
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/car/car_1}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/car/car_2} \tabularnewline 

\includegraphics[width=0.98\linewidth]{figures/teaser/park/ref} \tabularnewline
%\hspace{0.01em}

%\includegraphics[width=0.16\linewidth]{figures/teaser/single_video_gen_4} 
%\includegraphics[width=0.16\linewidth]{figures/teaser/single_video_gen_6} 
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/park/1}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/park/32}
\includegraphics[width=0.32\linewidth, height=0.08\textheight]{figures/teaser/park/25}
%\includegraphics[width=0.16\linewidth]{figures/teaser/park1201}



%\vspace{-1em}
\end{tabular}\hfill{}
\par\end{centering}
\caption{\label{fig:teaser} Images generated by SIV-GAN. Our model successfully operates in extremely low data regimes, generating new scene compositions with varying content and layout from a single image (first four rows) or a single video (last four rows). For example, from the single surfing image, SIV-GAN can synthesize layouts with a different position and configuration of waves varying the number of surfers in the scene; and for the single training video with a car on the road, it generates images without a car or with two cars . SIV-GAN is able to maintain the qualiS 
%the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene. change positions and configuration of waves in the see.   
%\caption{\label{fig:teaser} Images generated at different resolutions by SIV-GAN. Our model successfully operates in different extremely low-data regimes, including learning from a single video (first two rows) or a single image (last three rows), generating new scene compositions with varying content and layout. 
%For example, from the single training video with a car on the road, SIV-GAN generates images without a car or with two cars; and for the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene.  
%(Original samples are shown in grey or red frames.) \anna{caption should mention more strongly compositions of new scenes, and point out to high resolution images}
%One-Shot GAN images generated from a single video or a single image. Our model successfully operates in different one-shot settings, including learning from a single video (first two rows) or a single image (last three rows), generating new scene compositions with varying content and layout. 
%For example, from the single training video with a car on the road, One-Shot GAN generates images without a car or with two cars; for the single air balloon image, it can synthesize layouts with a different number and position of the balloons in the scene.  
%(Original samples are shown in grey or red frames.)
}
%\vspace{-1em}
\end{figure}

%- For Fig. 1, the caption should provide some additional explanation of the results. For the video, it is discussed in Section 4.3, but since the figure is at the beginning, it is better to give the reviewer directly the text that explains the quality of the results. You might move the figure also to page 2, if the caption gets longer.

==> rebuttal/figures/bus.tex <==
\begin{figure}[t]
\begin{centering}
\setlength{\tabcolsep}{0.1em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
%\vspace{-1em}
\hfill{}%
\begin{tabular}{@{\hskip -0.70in}c@{\hskip -0.0in}c@{\hskip -0.00in}c@{\hskip -0.00in}c@{\hskip -0.70in}}


\rotatebox{90}{\hspace{-.5ex}\begin{tabular}{c} \small SinGAN \\ \small ~\cite{Shaham2019SinGANLA}\end{tabular}}&
\includegraphics[width=0.25\linewidth, height=0.06\textheight]{figures/qual_single_video/bus_res_s1}~ & 
\includegraphics[width=0.25\linewidth, height=0.06\textheight]{figures/qual_single_video/bus_res_s2}~ & 
\includegraphics[width=0.25\linewidth, height=0.06\textheight]{figures/qual_single_video/bus_res_s3} 
\tabularnewline
\rotatebox{90}{\hspace{-.9ex}\begin{tabular}{c} \small One-Shot \\ \small GAN\end{tabular}}&
\includegraphics[width=0.25\linewidth, height=0.06\textheight]{figures/qual_single_video/bus_res_o1}~ &
\includegraphics[width=0.25\linewidth, height=0.06\textheight]{figures/qual_single_video/bus_res_o3}~ & 
\includegraphics[width=0.25\linewidth, height=0.06\textheight]{figures/qual_single_video/bus_res_o4} 

\end{tabular}\hfill{}
\par\end{centering}
%\vspace{-0.5em}
\caption{\label{fig:qual_video} Images generated from a video clip with a bus.
 }
\vspace{-1em}
\end{figure}

==> rebuttal/tables/single_video_abl.tex <==







\begin{table} [t]
	\centering
	\begin{minipage}{.55\linewidth}

		\setlength{\tabcolsep}{0.04em}
		\renewcommand{\arraystretch}{0.8}
		\centering
		

\vspace{-0.3ex}
\begin{tabular}{c|c|c}
	{\footnotesize{} Method } &  {\footnotesize{} SIFID $\downarrow$}  &   \footnotesize{} Dist. to train   \tabularnewline
	
	\hline 	\hline 	
	
	{\footnotesize{} Baseline}  & \footnotesize{1.8}     &  \color{darkred} \footnotesize{0.11}  \tabularnewline
	
	
	{\footnotesize{} Layout br.}  & \color{darkred}   \footnotesize{5.2}   &  \footnotesize{0.29} \tabularnewline
	
	{\footnotesize{} Content br.}   & \color{darkred}   \footnotesize{5.4}   &   \footnotesize{0.31}  \tabularnewline		
		{\footnotesize{} 2-branch $D$}  & \footnotesize{2.4}  &  \color{darkred} \footnotesize{0.13} \tabularnewline
	{\footnotesize{} 2-branch $D$+DR}  & \footnotesize{3.3}  &  \footnotesize{0.24} \tabularnewline	
\end{tabular}

\caption{Single Video setting.}
\label{rebuttal:sin_video} %

		
	%	\vspace{+0.9ex}
	\end{minipage}%
\begin{minipage}{.45\linewidth}
		\setlength{\tabcolsep}{0.04em}
	\renewcommand{\arraystretch}{0.8}
	\centering
	
%	\vspace{-0.4ex}
\begin{tabular}{@{\hskip -0.00in}c@{\hskip +0.02in}|@{\hskip -0.01in}c@{\hskip -0.0in}|@{\hskip -0.0in}c@{\hskip -0.01in}}

	{\footnotesize{} Method } &  {\footnotesize{} SIFID$\downarrow$}  &  {\footnotesize{} LPIPS$\uparrow$}   \tabularnewline
	
	\hline 	\hline 	
	
	  \footnotesize{} {SinGAN [33]} & \footnotesize{0.15}    &  \footnotesize{0.22}  \tabularnewline
	  
	  \footnotesize{} {~~~~~ + DR} & \footnotesize{0.17}    &  \footnotesize{0.22}  \tabularnewline	  \hline
	
	
	\footnotesize{} {FastGAN [1]}   & \footnotesize{0.14}  &   \footnotesize{0.14}  \tabularnewline		
	
		  \footnotesize{} {~~~~~ + DR} & \footnotesize{0.15}    &  \footnotesize{0.14}  \tabularnewline	%  \hline \hline
		  
	%\footnotesize{} {One-Shot GAN}   & \footnotesize{5.4}  &   \footnotesize{0.31}  \tabularnewline		

	%\footnotesize{} {~ -DR, +minibatch D} & \footnotesize{1.8}    &  \footnotesize{0.11}  \tabularnewline		 

\end{tabular}
%\vspace{0.4ex}
\caption{Single Image setting.}
\label{rebuttal:sin_image} %

\end{minipage}
\vspace{-4.0ex}
\end{table}













==> tables/comparison_single_image.tex <==
\begin{table}[t]
\vspace{-1em}
	\setlength{\tabcolsep}{0.15em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cc|c|c|c}
		\multirow{2}{*}{\normalsize{} Method } &  \multicolumn{2}{c|}{\small{} SIFID \cite{Shaham2019SinGANLA}} & \multirow{2}{*}{\small{} LPIPS$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel~$\uparrow$ }  \tabularnewline
		& \footnotesize{best}~$\downarrow$ & \footnotesize{mean}~$\downarrow$ & & & {\small{} Diversity } \tabularnewline
		
		\hline 	 \hline 	
		
		{\small{} SinGAN \cite{Shaham2019SinGANLA} } & \small{0.09}  & \small{0.15}  &  \small{0.22} & \small{0.75} & \small{0.52}  \tabularnewline

		
		{\small{} 1ConSinGAN \cite{Hinz2020ImprovedTF} } & \small{0.06}  & \small{0.08}  &    \small{0.24} & \small{0.73} & \small{0.50}  \tabularnewline
		
		{\small{} FastGAN \cite{anonymous2021towards} } & \small{0.11}  & \small{0.14} & \small{0.15} & \small{0.81} & \small{0.48}  \tabularnewline		
		
		{\small{} One-Shot GAN } & \textbf{\small{0.05}}  & \textbf{\small{0.06}} & \textbf{\small{0.28}} & \textbf{\small{0.67}} & \textbf{\small{0.57}}  
		
	\vspace{-0.5em}
		\end{tabular}
		\caption{Comparison with other methods on Places dataset in the Single Image setting.}
	\label{table:comp_single_image} %
	\vspace{-0.5em}
\end{table}


==> tables/comparison_single_image_fid.tex <==
\begin{table}[t]
	\vspace{-1em}
	\setlength{\tabcolsep}{0.7em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cccc}
		\multirow{2}{*}{\normalsize{} Method } &  \multicolumn{4}{c}{\normalsize{} SIFID ~$\downarrow$}  \tabularnewline
		& \footnotesize{$\frac{H\times W}{4}$\cite{Shaham2019SinGANLA}} & \footnotesize{$\frac{H\times W}{8}$} & \footnotesize{$\frac{H\times W}{16}$} & \footnotesize{$1\times 1$} \tabularnewline
		
		\hline 	 \hline 	
		
		{\small{} SinGAN \cite{Shaham2019SinGANLA} } & \small{0.15}  & \small{2.55}  &  \small{19.3} & \small{1370}  \tabularnewline

		
		{\small{} ConSinGAN \cite{Hinz2020ImprovedTF} } & \small{0.08}  & \small{1.75}  &    \small{18.9} & \small{1220}  \tabularnewline
		
		{\small{} FastGAN \cite{anonymous2021towards} } & \small{0.14}  & \small{2.83} & \small{15.9} & \small{1020}  \tabularnewline		
		
		{\small{} One-Shot GAN } & \textbf{\small{0.06}}  & \textbf{\small{1.09}} & \textbf{\small{14.4}} & \textbf{\small{880}}  

		\end{tabular}
		\vspace{-0.5em}
		\caption{Comparison with other methods in the Single Image setting using SIFID at different InceptionV3 layers.}
	\label{table:comp_single_image_fid} %
		\vspace{-1em}
\end{table}


==> tables/diversity_ablations.tex <==
\begin{table}[t]
	\vspace{-0.5em}
	\setlength{\tabcolsep}{0.1em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|c|c|c|c}
		\multirow{2}{*}{\small{Regularization} } & \multirow{2}{*}{\normalsize{} SIFID~$\downarrow$} & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel ~$\uparrow$}  \tabularnewline
        & & & & \small{} Diversity \tabularnewline
		
		\hline 	\hline 	
		
		{\normalsize None} &  \textbf{\small{0.045}}  &  \small{0.02} & \small{0.99} & \small{0.25}  \tabularnewline

		{\normalsize{} zCR \cite{zhao2020improved} } & \small{0.050}   &  \small{0.02} & \small{0.98} & \small{0.26}  \tabularnewline
		
		{\normalsize{} DS\cite{Yang2019DiversitySensitiveCG}   } & \small{0.048}  &  \small{0.08} & \small{0.88} & {\small{0.33}} \tabularnewline	
	

		%{\normalsize{} DS\cite{Yang2019DiversitySensitiveCG} ($G$ feat.)  } & \small{0.07}  &  \small{0.23} & \small{0.71} & {\small{0.53}} \tabularnewline	
		
			{\normalsize{} DR (im. space)   } & \small{0.066}  &  \small{0.13} & \small{0.84} & {\small{0.45}} \tabularnewline			
		
		{\normalsize{} DR   } & \small{0.063}  &  \small{0.24} & \small{0.72} & {\small{0.53}} \tabularnewline
				
		{\normalsize{} DR + FA   } & \small{0.064}  &  \textbf{\small{0.28}} & \textbf{\small{0.67}} & \textbf{\small{0.57}} 

		\end{tabular}
		\vspace{-0.5em}
		\caption{Ablation on diversity regularization techniques. }
	\label{table:ablation_diversity} %
		\vspace{-1em}
\end{table}


==> tables/main_ablations.tex <==
\begin{table}[t]

\vspace{-1em}
	\setlength{\tabcolsep}{0.2em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\begin{tabular}{c|cc|c|c|c}
		\multirow{2}{*}{\small{} Method } & \multicolumn{2}{c|}{\small{} SIFID~$\downarrow$}  & \multirow{2}{*}{\small{} LPIPS~$\uparrow$ } & \multirow{2}{*}{\small{} MS-SSIM~$\downarrow$} & {\small{} Pixel~$\uparrow$ }  \tabularnewline
		& \footnotesize{}  \footnotesize{$\frac{H\times W}{4}$} & \footnotesize{}  \footnotesize{$\frac{H\times W}{16}$} & & & \small{} Diversity   \tabularnewline
		
		\hline 	\hline 	
		
		{\small{} Baseline  } & \textbf{\small{0.04}} & \textbf{\small{6.9}}  &  \color{darkred}\small{0.07} & \color{darkred} \small{0.91} & \color{darkred} \small{0.31}  \tabularnewline
		
		{\small{} Layout br.   } & \small{0.16}   & \small{18.9}  & \textbf{ \small{0.33}} & \textbf{\small{0.63}} & \textbf{\small{0.58}}  \tabularnewline
		
		{\small{} Content br.   } & \small{0.08} & \small{17.5}  &  \small{0.28} & \small{0.68} & \small{0.56}  \tabularnewline
		
		{\small{} Full model   } & \small{0.06} & \small{14.4} &  \small{0.28} & \small{0.67} & \small{0.57}  \tabularnewline
	
		\end{tabular}
	\vspace{-0.5em}
	\caption{Ablation on the proposed discriminator structure on Places dataset in the Single Image setting. Indicators of collapsed diversity or poor quality are marked in red. 
	% when other methods passed 100.
}
\vspace{-0.5em}
\label{table:main_ablation} %

\end{table}


==> tables/manipulation.tex <==
\begin{table}[t]

	\setlength{\tabcolsep}{0.4em}
	\renewcommand{\arraystretch}{1.30}
	\centering
	\vspace{-0.9em}
	\caption{Comparison to image manipulation methods \cite{dong2022incremental,zhang2020deep} on DAVIS-YFCC100M in the Single Image setting.}
	\vspace{-0.9em}
	\begin{tabular}{c|c|c|c}

		\normalsize Approach & {\small SIFID~$\downarrow$}  & {\small LPIPS~$\uparrow$ } & Dist. to train  \tabularnewline

		
		\hline 	\hline 	
		

		\normalsize Image manipulation \cite{dong2022incremental,zhang2020deep} & \textbf{\small {{0.07}}}  &  \small {{0.19}}  &  \small {{0.18}}  \tabularnewline
		\normalsize SIV-GAN & \small {{0.08}}  &  \textbf{\small {{0.33}}} &  \small {{0.37}}
		 
	
		\end{tabular}
\label{tab:manipulation} %
	\vspace{-0.9em}

\end{table}


==> tex/ethics.tex <==
\section*{Ethics Statement}
\label{sec:Ethics}

All the authors of this work adhered to the ICLR Code of Ethics at the time of preparing the submission. 
We have made our best effort to uphold high standards of scientific excellence, avoid harm, discrimination, and dishonesty. All the experiments presented in the paper are conducted on publicly available datasets with a granted right for research-purposed usage.
Our organization is carbon neutral so that all its activities including research activities do no longer leave a carbon footprint. This also includes our GPU clusters on which the experiments have been performed.


The method presented in this work allows high-quality image synthesis in extremely low data regimes. Our model allows generating novel scene compositions requiring only a single image or video for training.
This ability can be potentially utilized in different applications, ranging from AI-based content editing to data augmentation of limited domains. 
For the content creation applications, similarly to other data-driven editing tools and graphical engines, a potential concern of misuse is the arising possibility for data manipulation. 
Photorealistic fake images synthesized by GANs may be presented as real photography in the media coverage, which may lead to negative societal outcomes. 
For the data augmentation, our model trained on rare samples can be used to generate more examples of underrepresented data, thus upsampling its proportion in the original data collection. This step will help to weaken the bias of datasets, providing more fairness in data coverage.


%For the latter, the potential concerns of misuse of our work fall into the same category as for other graphical engines and image synthesis tools. Such include arising possibilities for data manipulation, deepfakes, and other forms of misinformation. \anna{ideally extend this part a bit more}


%Our model can generate novel scene compositions, that differ from the original example, but preserve the realism of layouts and 

%This way, our algorithm contributes to existing generative models from the perspective of data efficiency. 
%\anna{not clear what you want to say here} The potential impact of this line of research is broadening the scope of GAN applications to various practical domains. 
%Therefore, the potential concerns of misuse of our work fall into the same category as for other graphical engines and synthesis tools. Such include arising possibilities for data manipulation, deepfakes, and other forms of misinformation. \anna{ideally extend this part a bit more}

==> tex/extensions.tex <==
\newpage
\onecolumn
~
\vspace{0.7cm}

\begin{center}
\section*{\label{sec:Extensions}Summary of extensions over a previous publication}
\end{center}
\vspace{0.5cm}

\begin{large}

We thank the editors and reviewers for considering this manuscript. %This work presents an extended version of our results that were presented at the CVPR 2021 workshop on Learning from Limited and Imperfect Data \cite{sushko2021one}. 
An early draft of the proposed idea was presented as a short 4-page workshop paper at the CVPR 2021 Workshop on Learning from Limited and Imperfect Data \cite{sushko2021one}.  
Compared to this short 4-page workshop paper, the current submission contains a significantly extended experimental evaluation of our model, new original ablation studies, as well as a more comprehensive description of the method and its positioning in the related work. The main differences for each section in the paper are summarized below.

\vspace{0.5cm}

\myparagraph{Introduction and related work.}
The preliminary workshop submission contained only a short introduction. It briefly introduced the single video training setup, explained high-level differences of our model from SinGAN \cite{Shaham2019SinGANLA} and FastGAN \cite{anonymous2021towards}, and enumerated our technical contributions. In contrast, in this manuscript we give a detailed introduction and provide a discussion of the recent related work. Thus, in the first two sections, the reader is now provided with a comprehensive positioning of our work with respect to prior single-image and few-shot image synthesis models, as well as image manipulation methods.

\vspace{0.5cm}

\myparagraph{Method.} The workshop paper provided only a short technical description of our content-layout discriminator and diversity regularization. Compared to this version, we extended the discussion on these components, introduced feature augmentation (FA) in Sec. \ref{sec:method_discriminator}, and added a new Sec. \ref{sec: train_det} describing our experimental setup and training details.


\vspace{0.5cm}

\myparagraph{Experiments.} The prior version had a reduced set of experiments, describing only the main results in the Single Image and Single Video settings (corresponding to our Tables \ref{table:comp_single_image} and \ref{table:comp_single_video}, Figs. \ref{fig:qual_image} and \ref{fig:qual_video}.) In our revised experimental section, we significantly extend the description of evaluation and add the comparisons to ConSinGAN model \cite{Hinz2020ImprovedTF} and image manipulation methods \cite{dong2022incremental, zhang2020deep} (Table \ref{tab:manipulation} and Fig. \ref{fig:manipulation}). Moreover, we provide a thorough ablation study  of our model in Sec. \ref{sec:exp_ablations}, including the new Tables \ref{table:main_ablation}, \ref{table:ablation_diversity}, \ref{table:lambda_dr}, \ref{table:N_low_level}, and the new Figs. \ref{fig:correlation}, \ref{fig:con_lay_embeddings}, \ref{fig:qual_ablations_d}, \ref{fig:fa}, \ref{fig:N_low_level}.

\vspace{0.5cm}

In conclusion, compared to the previous 4-page workshop paper, the current manuscript with 12 pages provides significantly extended original content.
%, which we find to fulfil the IEEE TIP requirement for a ``clearly identifiable benefit to the research community in comparison to the already published conference paper''.



\end{large}

\vspace{0.7cm}




==> tex/method.tex <==
\section{One-Shot GAN}
\label{sec:method}
\input{figures/model_overview}

%model motivation, overview of the model 

In this section, we present our One-Shot GAN model, which in comparison to previous methods~\cite{Shaham2019SinGANLA,Hinz2020ImprovedTF,anonymous2021towards}, can work in different one-shot regimes (single image and single video) and is designed not only to learn the internal patch-based distribution, but also to capture the  high-level content of the image and global layout coherency. The key ingredients of One-Shot GAN is the novel design of the two-branch discriminator (Sec.~\ref{sec:method_discriminator}) and the introduced diversity regularization for one-shot image synthesis (Sec.~\ref{sec:method_DR}).

\subsection{Content-Layout Discriminator} \label{sec:method_discriminator}

One of the challenges of training the GAN model in the one-shot setting regime is the problem of overfitting to the original sample. In many cases the model can simply memorize the original training image, and its augmentations (if used during the training). To avoid the memorization effect, \cite{Shaham2019SinGANLA,Hinz2020ImprovedTF} proposed to learn the internal patch-based distribution by using a hierarchy of patch-GANs \cite{isola2017image,Li2016PrecomputedRT} at different scales. Because the employed patch-GANs have small receptive fields and limited capacity, it prevents them from memorizing the overall image. However, as a downside those models can only synthesize images of low-level diversity tuned to the chosen minimal size and number of scales.  If the image contains a more complex scene, they quite often generate images with incoherent global layouts (see Fig.~\ref{} \anna{need to show the example here to proof the point}), and thus do not generalize well to other settings, such as learning from a single video (see Table~\ref{table:comp_single_video}).  

We therefore introduce an alternative solution to overcome the memorization effect but still to produce images of high-level diversity. In particular, we propose a two-branch discriminator, disentangling its decision about the content and layout realism of the image into separate branches. Note that the branching of the discriminator happens after intermediate feature layers; this is done in order to learn the relevant representations for building the content and layout branches.  
The discriminator judging the internal content distribution irrespective from the scene layout realism, and vice versa, enables the generator to synthesize images with varying content and global layouts.
In order to also preserve the good low-level details of the generated images, such as textures, we additionally ask the discriminator to make the real/fake decision based on the feature representations extracted at the lower intermediate layers (before branching). 
The loss of the new discriminator $D$ is then computed by taking the decisions from the content branch $D_{content}$, the layout branch $D_{layout}$ and from the low-level features of the discriminator $D_{low-level}$:
\begin{align}
& \mathcal{L}_{D}  = \mathcal{L}_{D_{low-level}} + \mathcal{L}_{D_{content}} + \mathcal{L}_{D_{layout}}, \label{eq:loss_d}
\end{align} 
where $\mathcal{L}_{D_{*}} = -\mathbb{E}_x[\log D_{*}(x)]- \mathbb{E}_z[\log (1-D_{*}(G(z)))]$.
The architecture of the content-layout discriminator is depicted in Figure \ref{fig:model_over}, and its branches are described below.

\paragraph{Content branch}
The decision of the content branch of the discriminator should be based upon the internal content of the image - the fidelity of "objects" composing the image, independent of their spatial location in the image layout.
%\textit{content} -- the presence of elements/parts composing the object, and \textit{location} -- the spatial placement and arrangement of these parts.
Let the dimension of the input feature map $F_{input}$ of the content branch be $H\times W\times C$, where $H$, $W$, $C$ are the height, width and channels of the feature map. Note that the spatial resolution $H\times W$ captures spatial information and channels $C$ encode feature representations. Upon removing the spatial information from the channels, the network is induced to respond to the content features encoded in different channels irrespective of their spatial location. Hence, we propose to aggregate the spatial information $H\times W$ across the channels $C$ in order to remove the layout information and allow the network to make its decisions based on the feature representation encoded in spatially aggregated channels $F_{content}$ with size $1\times\ 1\times C$. For the spatial aggregation we use average pooling ...

\anna{mention here feature augmentations specific to the content branch to encourage content diversity}
\anna{formalize discriminator content loss, mention loss for intermediate layers}

\paragraph{Layout branch}

\anna{mention here feature augmentations specific to the layout branch to encourage layout diversity}
\anna{formalize discriminator layout loss, mention loss for intermediate layers}

%\paragraph{Feature and data augmentations}
%data augmentations
%feature augmentations for different branches 


full loss for new 2-branch D

\subsection{Diversity Regularization} \label{sec:method_DR}

To improve the variability of the generated image samples, we propose to add diversity regularization (DR) loss term $\mathcal{L}_{DR}$ to the One-Shot GAN objective.
Prior work of \cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR} also proposed to use diversity regularization for GAN training, but mainly to avoid mode collapse and assuming the availability of a large set of training samples. The regularization of \cite{Yang2019DiversitySensitiveCG} aimed to encourage the generator to produce different outputs depending on the input latent code, in such way that the generated samples with closer latent codes should look more similar to each other, and vice versa.
In contrast, our diversity regularization is tuned for one-shot image synthesis. Assuming that in the one-shot mode we are operating in one semantic domain, the generator should produce images that are in-domain but more or less equally different from each other and substantially diverse form the original training sample. In the one-shot image synthesis setting, the perceptual distance of the generated images should not be dependent on the distance between their latent codes.
Thus, we propose to encourage the generator to produce perceptually different image samples independent of their distance in the latent space. Mathematically, the new diversity regularization is expressed as follows:
\begin{align}
\mathcal{L}_{DR} (G) = \mathbb{E}_{z_1,z_2}\big[\frac{1}{L}\sum_{l=1}^{L}\|G^{l}(z_1)-G^{l}(z_2)\|)\big], \label{loss_DR}
\end{align}
where $\|\cdot\|$ denotes the norm, $G^{l}(z)$ indicates a feature extracted from $l$th layer of the generator $G$ given input $z$, and $z_1, z_2$ are randomly sampled latent codes in the batch, i.e. $z_1,z_2 \sim N(0,1)$.
By regularizing generator to maximize Eq.~\ref{loss_DR}, we force the generator to produce diverse outputs for different latent codes $z$.
Note that, in contrast to \cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR}, we compute the distance between samples in the feature space of the generator. Computing the sample distance in the feature space enables more meaningful diversity of the generated images. Different layers of the generator capture different semantics of the image, inducing both high-level and low-level diversity in samples.
Computing the sample distance directly from the generator outputs (in the pixel space), as in \cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR}, i.e. $\|G(z_1)-G(z_2)\|$, in our experiments leads to limited diversity and also worse quality of the generated samples.

An overall One-Shot GAN objective can be written as:
\begin{align}
\min_{G} \max_{D} \hspace{0.5em} \mathcal{L}_{GAN} (G,D) - \lambda \mathcal{L}_{DR} (G), \label{loss_full}
\end{align}
where $\lambda$ controls the strength of the diversity regularization and $\mathcal{L}_{GAN}$ is the adversarial loss.
%The adversarial loss is expressed as: 
%\begin{align*}
%\mathcal{L}_{GAN} (G,D) = \mathbb{E}_x[\log D(x)] + \mathbb{E}_z[\log (1-D(x,G(z)))],
%%$\label{eq:loss_gan}
%\end{align*}
%where the two-branch discriminator $D$ aims to distinguish between real $x$ and generated $G(z)$ images based on their content and layout realism.
The proposed diversity regularization is simple, can be easily integrated into different GAN objectives, and highly-effective for the one-shot image synthesis task, where previous diversity regularizations~\cite{Yang2019DiversitySensitiveCG,Zhao2020ImprovedCR} fail (see Sec.~\ref{sec:exp_sin_image} and Table~\ref{table:ablation_diversity}).

\subsection{Implementation and Training}

architecture details, training details

==> tex/rebuttal.tex <==
\newpage
\onecolumn
~
\vspace{0.7cm}

\begin{center}
\section*{\label{sec:Rebuttal}Response to the reviewers}
\end{center}
\vspace{0.5cm}

\begin{large}

We thank the AE and the reviewers for their valuable comments. According to the suggestions of the AE
and reviewers, we have revised our paper, providing additional experiments and adding more precise discussions of our contributions. Below are the detailed responses to the concerns raised by the reviewers.

\vspace{0.5cm}

\myparagraph{Response to Reviewer 1:}


\vspace{0.4cm}

\myparagraph{R1: Can you control the position where the added objects to the scene? Or is it just random? I didn't see that interactive information from fig.2. The paper needs a discussion regarding using existing tools for image manipulation (inpainting, object blending) instead of a GAN model.}

\vspace{0.1cm}

\myparagraph{Answer:} First, we want to clarify that we do not address interactive image editing like in-painting or object blending where a user manually defines the image editing operations like masking an object that should be removed. There is therefore no interactive component that defines which and where objects should be added. In this work, we address the research question how a GAN can be trained on a single image or frames of a single video, which then generates plausible but diverse variants of the training image(s). We therefore compare to other GANs that are trained on one or few images. Although the network has no explicit information or user input where objects in the image are, our approach is able to preserve objects, removes them or adds more of them, but it also changes the scene in a plausible way. This is an astonishing result. The images are generated by sampling randomly from the noise vector. The approach can thus automatically generate infinitely many novel examples from a single training image or video. This is beneficial for practical applications, e.g., recognizing rare species or objects of which only one image or video exists. We revised the introduction (Sec.~\ref{sec:introduction}) and added additional explanations.

\myparagraph{New experiment:} We agree that in such a scenario a user could also manually generate a few variants of the training image using image inpainting or object blending. Note that this requires an additional manual effort by masking objects, while our approach generates the new images automatically using only an image or a video as input without any annotations. Nonetheless, we added a comparison between our model and state-of-the-art methods for image inpaiting \cite{dong2022incremental} and object blending \cite{zhang2020deep}. For the comparison, we pick 15 images from DAVIS-YFCC100M and supplement them with pixel-wise masks of foreground objects. The image manipulation is then performed in two steps: 1) remove a foreground object using image inpainting; 2) blend the object at different random locations within a scene. The results are presented in Fig.~\ref{fig:manipulation} and Table~\ref{tab:manipulation}. We note the image manipulation methods can exhibit inpaiting distortions and produce unrealistic objects at new locations. Furthermore, these methods allow to achieve only reduced diversity compared to SIV-GAN. We also note that the synthesis capability of our method is much wider than in-painting or blending: our method can actually create new structures, e.g., buses of different lengths in Fig.~\ref{fig:qual_video}.


%%%% OLD ANSWER TO R1
%\myparagraph{Answer:} We note that a misunderstanding must have happened. We are sorry if this happened due to the lack of clarity in our presentation. In this paper we study unconditional image synthesis, not controllable image editing.  In our task, each image is generated from a noise vector and is not conditioned on any other ``interactive'' information. Thus, no additional parameters explicitly controlling the spatial position of located objects or layout of background are provided to the model.
%\myparagraph{}The advantage of \textit{unconditional} image synthesis is its small manual overhead. Our model does not require a user to provide an additional input (e.g., pixel-wise mask) for each generated image. Thus, after training, our model allows to automatically sample infinitely many novel examples. This can be beneficial for practical applications dealing with generation of data augmentation, where the requirements for the quality, diversity and amount of generated samples can be high. We revised the introduction (Sec. 1) and added additional explanations.
%\vspace{0.4cm}
%\myparagraph{R1: The paper needs a discussion regarding using existing tools for image manipulation (in-painting, object blending) instead of a GAN model.}
%\vspace{0.1cm}
%\myparagraph{Answer:} We argue that our initial goal is not controllable image editing. The ability to remove or duplicate objects is not a part of our original motivation, but rather an interesting result that we observed with our model. Instead, the focus of our paper is \textit{unconditional image synthesis}. 
%\myparagraph{}From a technical perspective, our task is significantly different from image editing. Image editing methods, such as in-painting or blending, assume at least two inputs: an image, and an indication of which pixels should be edited. The image area outside of the edited pixels should be preserved in these methods. In contrast, our method never assumes any object information as input: it just needs images during training, and needs only a noise vector during inference. Moreover, our model does not aim to preserve any pixels from the original image, but aims to achieve high synthesis diversity, thus avoiding copying image areas of given images. 
%\myparagraph{New experiment:} Nonetheless, we agree that in extremely low data regimes our task visually reminds image editing. \anna{I think it's better still argue that the tasks are sufficiently different, but here we can still compare due to low annotation effort required and that we can use the GT masks from the dataset. Otherwise it reads as if we contradict our statement in the above paragraph} Thus, we now provide a comparison between our model and state-of-the-art methods for image inpaiting \cite{dong2022incremental} and object blending \cite{zhang2020deep}. For the comparison, we pick 15 images from DAVIS-YFCC100M and supplement them with pixel-wise masks of foreground objects. The image manipulation in then performed in two steps: 1) remove a foreground object using image inpainting; 2) blend the object at different random locations within a scene. The results are presented in Fig. 10 and Table 7. We note the image manipulation methods can exhibit inpaiting distortions and produce unrealistic objects at new locations. Furthermore, these methods allow to achieve only reduced diversity compared to SIV-GAN. We also note that the synthesis capability of our method is much wider than in-painting or blending: our method can actually create new structures, e.g., buses of different lengths in Fig. 5.
%\myparagraph{}We note that while achieving stronger results, SIV-GAN still does not utilize the provided pixel-wise mask in this experiment. In practice, requiring segmentation masks of foreground objects and interactive selection of new image areas for blending can be restrictive, which can make our model favourable in some applications, such as generating more images for data augmentation.
%\myparagraph{}Considering our clarifications and extensions above, we invite R1 to re-assess our work.

\vspace{0.4cm}

\myparagraph{R1: It is not clear how does authors make sure the content branch different from layout branch.}

\vspace{0.1cm}
 
\myparagraph{Answer:} The content and layout branches are induced to assess different aspects of an input image, because they receive the intermediate representation $F(x)$ squeezed in two different ways (along the channel or spatial dimensions). Let us consider the following example: take an image with air balloons from Fig.~\ref{fig:teaser} (1st row), and paste one more yellow balloon instead of a dark blue balloon. This transformation would not change the feature representation of the image in the layout embedding, since the layout map is insensitive to the changes in object colors. In contrast, the content representation would be changed, since the content representation can detect the absence of a dark blue balloon object. Therefore, the same image may appear realistic for one branch and unrealistic for another branch. In addition, the two branches employ different Feature Augmentation (FA).
%Note that the original representation $F(x)$ cannot be reconstructed from these two. Thus, 

\myparagraph{}We demonstrate the difference between branches quantitatively in Table~\ref{table:main_ablation}, qualitatively in Fig.~\ref{fig:qual_ablations_d}, and in a new experiment in Fig.~\ref{fig:con_lay_embeddings}. The ablation in Table~\ref{table:main_ablation} demonstrates that the model achieves different performance with different branches, and the best performance is achieved only when both branches are used. Fig.~\ref{fig:qual_ablations_d} demonstrates our visual intuition on what the content and layout branches learn. 

\myparagraph{New experiment:} In Fig.~\ref{fig:con_lay_embeddings} we show the feature distances in the embeddings of SIV-GAN content and layout branches. For this, we train SIV-GAN on single videos ``bus'' and ``parkour'' from the DAVIS dataset \cite{pont20172017} and take the discriminators. The plots show the feature distances measured between the real middle frame and other real frames of the same video sequence. The illustrated distances behave differently for the content and layout branches. Firstly, the layout embedding distances (solid red) between ``bus'' frames are notably lower than for the ``parkour'' video. This is in line with the perceptual judgement (note a camera direction movement for the ``parkour'', while the ``bus'' is always captured from the same angle). In contrast, the content embeddings values for the two sequences (solid blue lines) have similar ranges. Secondly, as video frames inside the short videos depict similar content (e.g.  same objects), the content embedding distances between frames of the same sequence (solid blue) are significantly lower than to middle frames of two different videos (dashed blue). This is not the case for layout embeddings, as the difference in layouts inside one video (solid red) can be almost as high as layout difference between frames of two different sequences (dashed red).


%\anna{I would add here Fig.C for explanation, that shows that learnt embeddings of 2 branches are different from each other. I think it makes quite a convincing argument for the reviewer}



\vspace{0.4cm}

\myparagraph{R1: It seems that this idea is highly similar to swap-autoencoder (NeurIPS 2020).	Can authors highlight more on the difference?}

\vspace{0.1cm}

\myparagraph{Answer:} We agree that prior work also explored multi-branch GAN architectures. Some works, including the Swapping Autoencoder \cite{Park2020SwappingAF}, separated ``content'' and ``style'' features in generators \cite{wu2019disentangling,huang2018multimodal}, aiming to achieve more control over synthesized images by separately varying content or style conditioning for generator. For example, the Swapping Autoencoder \cite{Park2020SwappingAF} uses one ``content'' and one ``style'' reference image to produce a new image. Their feature separation into a 1D-vector and a tensor with spatial dimensions is introduced to primarily improve the disentanglement. In their task, the generator has to be able to reconstruct the original image given its content and style features.

\myparagraph{}Our research direction is different. We aim to train a GAN given extremely limited data. We do not aim to reconstruct the original image because this would lead to memorization problems. In our task, the memorization happens on the side of discriminator, not generator. We thus carefully analyse what is required to prevent the \textit{discriminator} memorization, and develop two different branches to weaken the ability of discriminator to memorize the full image, but still to guide the generator towards realistically looking images. This could not be achieved with previous methods. We extended our related work section with this discussion.


%\myparagraph{}The difference of our idea to Swapping Autoencoder \cite{Park2020SwappingAF} is how and where the feature restriction is used. Swapping Autoencoder \cite{Park2020SwappingAF} aims to disentangle the texture and structure representations that are used as conditioning for the \textit{generator}. To learn the image manipulation task, the generator in \cite{Park2020SwappingAF} should be able to perfectly reconstruct the original image from these two representations. In case of a single training image, this solution would force the Swapping Autoencoder to memorize the original frame. In contrast, our solution is developed for the \textit{discriminator} to prevent the memorization issue. We never aim to reconstruct an image from given content or layout features, and apply only adversarial losses on these features. We added this comparison to the related work section.

\vspace{0.4cm}

\myparagraph{R1: It is not clear how authors use perceptual loss such as LPIPS to measure the quality of the generated images? Whether there is any bias in using LPIPS to measure?}

\vspace{0.1cm}

\myparagraph{Answer:} We use LPIPS to evaluate diversity, not quality. LPIPS can be regarded as a measure of perceptual distance between two images. The higher the LPIPS, the more different two images are perceptually. Thus, we sample 100 images from our trained generator and compute LPIPS between each of ($100\cdot99/2=4950$) image pairs. The final metric is taken as an average across all the pairs. This average LPIPS indicates the average diversity of an image generator, and is commonly used in other works on image synthesis \cite{Yang2019DiversitySensitiveCG,ojha2021few}. 



%\anna{maybe here cite another work than OASIS, to highlight that the metric is not introduced by us, as authors are visible to reviewers}

\myparagraph{}We are not aware of a significant bias while using LPIPS. In general, the LPIPS network is pre-trained on ImageNet, thus it is usually better suited for natural image domains. Moreover, it was designed to correlate with the perceptual human judgement, which is biased towards high-level image patterns. Nonetheless, we did not observe any significant biases compared to using other diversity measures, e.g., Pixel diversity (Tables 1,3-5).


\vspace{0.5cm}

\myparagraph{Response to Reviewer 2:}

\vspace{0.4cm}

\myparagraph{R2: While this paper also focus on synthesis for video and the authors claimed that "we aim to generate images and not temporally-coherent videos", I still think failing to generate temporally-coherent video is a drawback.}

\vspace{0.1cm}

\myparagraph{Answer:} We agree that generating temporally-coherent videos such as in \cite{tulyakov2018mocogan} is an interesting direction, but it is out of scope since it requires a very different network architecture than a GAN that generates images. The focus of this work is on training GANs for generating images in extremely low data regimes, i.e., one training image or few highly correlated images. For the latter case, we use a single video for two reasons: a) frames that are close in a video are highly correlated b) from a practical point it is the same effort to capture a single image or video, but it is difficult/infeasible to capture a similar scene or the same object at another point in time. Note that few-shot learning of GANs in the context of highly correlated images has not been studied before and the results show that previous GAN models for few-shot learning perform poorly in case of highly correlated images. We thus believe our model can advance the application of GANs to new practical domains. We revised the introduction, improved the explanation, and added an additional experiment.

%%% OLD R2 answer
%\myparagraph{Answer:} We are sorry if our presentation caused a confusion about our goals. Generating realistic videos utilizing temporal relations between frames, such as in \cite{tulyakov2018mocogan}, is a very different task from ours. We study \textit{unconditional image generation}, when a GAN is trained on \textit{unordered} collection of frames. 
%\myparagraph{}Our specific focus is on GANs in extremely low data regimes. A single video sequence is an interesting source of data for us for two reasons: 1) such data is easy to collect; 2) the correlation between image frames is much higher than in other few-shot datasets. The latter introduces a new challenging few-shot benchmark for training GANs, where training images are very similar to each other. Such scenarios can be interesting in practice%(e.g., pictures of manufacturing defects, medical images)
%, but prior GAN models could not successfully learn in this regime. Thus, in our work, video frames are considered as an interesting example of a dataset with very similar images, rather than temporally-coherent frames. We thus believe our model can advance the application of GANs to new practical domains. We revised our introduction and included better explanations.
%which can open their new applications. Let us consider the following example: take a few images of defects in a product at a manufacturing plant. Usually, such images look very similar to each other and differ only in tiny details. A practical task of a GAN model can be to generate data augmentation from this data.

\myparagraph{New experiment:} We conducted an additional experiment highlighting the impact of the similarity of the training images for few-shot learning (see Sec.~\ref{sec:exp_sin_vid} and Fig.~\ref{fig:correlation}). For this, we picked several videos from YFCC100M and varied the distance between the sampled frames by taking only each 1st, each 2nd, ..., each 10th frame (but always keeping the overall number of frames equal to 100). We observed that the previous few-shot method FastGAN suffers most from memorization when learning from a set of very similar images. Considering that the single video setup appears challenging for previous methods, we believe that it is an important few-shot benchmark for unconditional GANs.

%\anna{here I would add in the end that we think that generating temporally-coherent videos in one- and few-shot setting is an interesting future direction for our work. You can also mention that this is a more computationally resource demanding setting}

\vspace{0.4cm}

\myparagraph{R2: The main novelty of content-layout discriminator and diversity regularization seems to be not significant enough for an TPAMI paper.}

\myparagraph{Answer:} Let us share our perspective on the novelty aspect. We present an approach that for the first time is able to generate plausible and diverse images when it is trained on few images that are highly correlated. Neither one-shot nor few-shot GANs can handle such case as we show in the paper. We carefully analyse what is required to prevent memorization or mode collapse in such extremely low-data regimes. Our model also outperforms other approaches when it is trained on a single image. The impact of highly correlated training images on GANs has not been studied before and this is the first work that shows that it has a high impact. We thus think that this is an important contribution for understanding and analysing GANs in low-data regimes better.           


%%% OLD R2
%Let us share our perspective on the novelty aspect. 1) We acknowledge that the proposed methodology is conceptually simple. However, we think it can be considered an advantage that an uncomplicated approach solves the task effectively. 2) Our novelty also includes a new GAN benchmark and a novel analysis of GAN training on few-shot datasets with very similar images. We for the first time demonstrated the importance of average image similarity for few-shot GAN training (see new Sec. 4.2). Our method enables successful GAN learning in a new data regime, which can potentially open GAN application to data domains where GANs were not applied previously.


\end{large}

\vspace{0.7cm}




==> tex/reproducibility.tex <==
\section*{Reproducibility Statement}
\label{sec:Reproducibility}

The authors have made their best effort to ensure the reproducibility of the methods presented in this work. A complete description of our algorithmic proposals is presented in Sec.~\ref{sec:method}, and our experimental and evaluation settings are discussed in Sec.~\ref{sec:experiments}.
%\anna{should be a reference to the method section ?} 
%\anna{also say we describe the experimental and evaluation settings} 
An extended description of all architectural solutions, training details, including a detailed scheme of our networks is included in App.~\ref{sec:architecture}. To facilitate the usage of our models and the reproduction of our results, we will release publicly our training code and trained model weights, providing a complete list of images and videos used for experiments.
%\anna{you also use a combination of images/videos. so the supplementary should include the names or you should mention that you release them}

==> tex/resubmission.tex <==
\onecolumn
~
\vspace{0.7cm}

\setlength\parindent{0pt}

\begin{center}
\section*{\label{sec:Extensions}Summary of the previous review round.}
\end{center}
\vspace{0.5cm}

This manuscript has been previously submitted to IEEE Transactions on Pattern Analysis and Machine Intelligence. In line with the IEEE Transactions on Image Processing guidelines, we provide this supplementary material which includes the details on the previous review rounds and outlines how the feedback was incorporated into the new version of the paper. We also want to point out that there was a disagreement among the previous reviewers and one reviewer recommended to submit the manuscript to IEEE Transactions on Image Processing. In the following, we verbatim copied the reviews of the two rounds from IEEE Transactions on Pattern Analysis and Machine Intelligence and finally discuss how the final remarks after the second round have been addressed in the submitted manuscript.       


\vspace{0.5cm}

\myparagraph{Overview of the review rounds.}

Our paper was reviewed by two reviewers in two rounds. Reviewer 1 initially had concerns about the novelty of the paper and the motivation of the Single Video setting. After reading our response and the paper revision, Reviewer 1 recommended acceptance. Reviewer 2 initially expressed concerns about the applications of the method and asked questions on technical details and evaluation. Reviewer 2 misunderstood the paper and considered that the work is on image editing whereas the work is about unconditional image synthesis. Although we clarified this point in the response for the second round, Reviewer 2 still insisted that an `interactive component' for image editing is missing.   

%\vspace{0.5cm}
\myparagraph{Reviews after first round:}

\begin{displayquote}

\myparagraph{Reviewer: 1}

Recommendation: Author Should Prepare A Major Revision For A Second Review

\vspace{0.2cm}

Comments:

This paper aim to leverage the GAN network to  learn a model which is able to compose
new layouts, re-arrange objects in the scene, remove or duplicate instances, and change their shape and size.

After I read this paper, I do have a biggest question regarding the proposed method:
1. For object removal ? How well does existing in-painting method did ?  I don't see any comparisons on that.
For composite another object into the scene, how well does existing blending method did ?

2. Can you control the position where the added objects to the scene ?  Or it is just random ? I didn't see that interactive information from fig.2


I do have big questions regarding my 1st  question and 2nd question regarding using existing tool for manipulate the images rather than using single image gan method. I felt it needs a heavy discussion on that.

3. It is not clear how does authors make sure the content branch different from layout branch. Also, it seems that this idea is highly  similar to swap-autoencoder
"Swapping Autoencoder for Deep Image Manipulation" NeurIPS 2020

Can authors highlight more on the difference ?

4. It is not clear how authors use perceptual loss such as LPIPS to measure the quality of the generated images ? Whether there is any bias in using LPIPS to measure ?

\myparagraph{Reviewer: 2}

Recommendation: Author Should Prepare A Major Revision For A Second Review

\vspace{0.2cm}

Comments:

This paper proposed an unconditional generative model which learns from a single image or a video sequence. The main idea is to introduce content-layout discriminator and diversity regularization to enable synthesis of visually plausible, novel compositions of a scene, with varying content and layout. Experiments demonstrate the effectiveness of the proposed method.

This paper is an extension of short 4-page workshop paper. Overall, this paper is well-written. The authors also released the codes.

My concerns toward this paper are given as follows.

First, the main novelty of content-layout discriminator and diversity regularization seems to be not significant enough for an TPAMI paper. I would like to give an acceptance for an TIP paper.

Second, while this paper also focus on synthesis for video and the authors claimed that "we aim to generate images and not temporally-coherent videos", I sitll think failing to generate temporally-coherent video is a drawback.

\end{displayquote}

\myparagraph{Reviews after second round:}

\begin{displayquote}

\myparagraph{Reviewer: 1}

Recommendation: Accept With No Changes

\vspace{0.2cm}

Comments:

I appreciate the response, the authors have addressed my concerns, I would like to give an acceptance.

\vspace{0.2cm}

Additional Questions:

1. Which category describes this manuscript?: Practice / Application / Case Study / Experience Report

2. How relevant is this manuscript to the readers of this periodical? If you answer Not very relevant or Irrelevant please explain your rating under Public Comments below.: Very Relevant

1. Please evaluate the significance of the manuscript’s research contribution.: Excellent

2.  Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: See comments.

3. Is the manuscript technically sound? In the Public Comments section, please provide detailed explanations to support your assessment: Yes

1. Are the title, abstract, and keywords appropriate? If not, please comment in the Public Comments section.: Yes

4. How thorough is the experimental validation (where appropriate)? Please discuss any shortcomings in the Public Comments section.: Compelling experiments; clearly state of the art

2.  Does the manuscript contain sufficient and appropriate references?  Please comment and include additional suggested references in the Public Comments section.: References are sufficient and appropriate

If you are suggesting additional references they must be entered in the text box provided.  All suggestions must include full bibliographic information plus a DOI.


If you are not suggesting any references, please type NA.:

3.  Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? If not, please explain your answer in the Public Comments section.: Yes

4.  How would you rate the organization of the manuscript? Is it focused? Please elaborate with suggestions for reorganization in the Public Comments section.: Satisfactory

6. How is the length of the manuscript?  If changes are suggested, please make explicit recommendations in the Public Comments section.: About right

5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Easy to read

7. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): Yes, as part of the digital library for this submission if accepted

8. If yes to 7, should it be accepted: As is

Please rate the manuscript overall. Explain your choice.: Excellent


\myparagraph{Reviewer: 2}

Recommendation: Reject

\vspace{0.2cm}

Comments:

Personally, authors didn't address my previous comments in the right way. And I still cannot convince by authors response.

For example,
1. 'There is therefore no interactive component that defines which and where objects should be added'
For me, if there is no interactive component could define, then what's the real application for this paper ?
If authors claim that this is a theory paper, then what's the theory part ?

2.  I don't believe it is 'This is an astonishing result'. For me, this is totally over claim without any real application value.

3. If authors believe that ''This is an astonishing result'', please compare with all the existing Dalle2, stable diffusion methods since they can also do 1 image finetune such as dreambooth type of technology (I know dreambooth is not for 1 image but I mean similar)


4. In-painting doesn't need any precise mask, simple bursh already working very well. I still believe authors should compare.

\vspace{0.2cm}

Additional Questions:

1. Which category describes this manuscript?: Practice / Application / Case Study / Experience Report

2. How relevant is this manuscript to the readers of this periodical? If you answer Not very relevant or Irrelevant please explain your rating under Public Comments below.: Relevant

1. Please evaluate the significance of the manuscript’s research contribution.: Poor – This manuscript either has serious technical flaws, does not solve an important problem, or presents a variation of a well known technique.  It should not be published in TPAMI.

2.  Please explain how this manuscript advances this field of research and/or contributes something new to the literature.: Personally,  like I mentioned last time. I didn't see much value that paper could bring to the image composition use cases and also recent diffusion-based approaches has much better results than this paper a lot.

3. Is the manuscript technically sound? In the Public Comments section, please provide detailed explanations to support your assessment: No

1. Are the title, abstract, and keywords appropriate? If not, please comment in the Public Comments section.: Yes

4. How thorough is the experimental validation (where appropriate)? Please discuss any shortcomings in the Public Comments section.: Insufficient; clearly inferior to state of the art, or necessary tests are absent

2.  Does the manuscript contain sufficient and appropriate references?  Please comment and include additional suggested references in the Public Comments section.: Important references are missing; more references are needed

If you are suggesting additional references they must be entered in the text box provided.  All suggestions must include full bibliographic information plus a DOI.


If you are not suggesting any references, please type NA.:

3.  Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? If not, please explain your answer in the Public Comments section.: Could be improved

4.  How would you rate the organization of the manuscript? Is it focused? Please elaborate with suggestions for reorganization in the Public Comments section.: Could be improved

6. How is the length of the manuscript?  If changes are suggested, please make explicit recommendations in the Public Comments section.: About right

5. Please rate the readability of the manuscript. Explain your rating under Public Comments below.: Readable - but requires some effort to understand

7. Should the supplemental material be included? (Click on the Supplementary Files icon to view files): Does not apply, no supplementary files included

8. If yes to 7, should it be accepted:

Please rate the manuscript overall. Explain your choice.: Fair 

\end{displayquote}

\myparagraph{Incorporation of the feedback into the revision.}

\begin{itemize}
    \item \textbf{Reviewer 1.} The initial concerns of Reviewer 1 were addressed in the paper revision during the previous submission. After the revision, Reviewer 1 recommended acceptance with no further changes. 
    \item \textbf{Reviewer 2.} Our current submission addresses each of the comments of Reviewer 2 from the second round. Firstly, the writing of the paper now clearly outlines the difference of our method to image manipulation methods and mentions its advantages over image manipulation methods in some practical scenarios (Introduction on page 2) (comments 1-2). Secondly, we adjusted the wording of the claims to avoid concerns on over-claiming (comments 2-3). Thirdly, as suggested by Reviewer 2, we added a comparison of our model to recent image manipulation methods, including image in-painting (Sec. \textit{IV-D}, Fig. 11, Table \textit{VII}) (comment 4).
\end{itemize}


\begin{comment}


\myparagraph{Reviewer 1 -- first round:}

This paper proposed an unconditional generative model which learns from a single image or a video sequence. The main idea is to introduce content-layout discriminator and diversity regularization to enable synthesis of visually plausible, novel compositions of a scene, with varying content and layout. Experiments demonstrate the effectiveness of the proposed method. This paper is an extension of short 4-page workshop paper. Overall, this paper is well-written. The authors also released the codes. My concerns toward this paper are given as follows.
\begin{itemize}
    \item First, the main novelty of content-layout discriminator and diversity regularization seems to be not significant enough for an TPAMI paper. I would like to give an acceptance for an TIP paper.
    \item Second, while this paper also focus on synthesis for video and the authors claimed that "we aim to generate images and not temporally-coherent videos", I still think failing to generate temporally-coherent video is a drawback. 
\end{itemize}




\vspace{0.5cm}


\myparagraph{Reviewer 1 -- second round:}

I appreciate the response, the authors have addressed my concerns, I would like to give an acceptance.

\vspace{0.5cm}

\myparagraph{Reviewer 2 -- first round:}


This paper aim to leverage the GAN network to  learn a model which is able to compose new layouts, re-arrange objects in the scene, remove or duplicate instances, and change their shape and size. After I read this paper, I do have a biggest question regarding the proposed method:
\begin{itemize}
    \item For object removal ? How well does existing in-painting method did ?  I don't see any comparisons on that. For composite another object into the scene, how well does existing blending method did?
    \item Can you control the position where the added objects to the scene ?  Or it is just random ? I didn't see that interactive information from fig.2. I do have big questions regarding my 1st  question and 2nd question regarding using existing tool for manipulate the images rather than using single image gan method. I felt it needs a heavy discussion on that.
    \item It is not clear how does authors make sure the content branch different from layout branch. Also, it seems that this idea is highly  similar to swap-autoencoder ``Swapping Autoencoder for Deep Image Manipulation'' NeurIPS 2020. Can authors highlight more on the difference?
    \item It is not clear how authors use perceptual loss such as LPIPS to measure the quality of the generated images ? Whether there is any bias in using LPIPS to measure ?

\end{itemize}

\vspace{0.5cm}

\myparagraph{Reviewer 2 -- second round:}


Personally, authors didn't address my previous comments in the right way. And I still cannot convince by authors response.
For example,
\begin{itemize}
    \item For me, if there is no interactive component could define, then what's the real application for this paper? If authors claim that this is a theory paper, then what's the theory part ?
    \item I don't believe it is ``This is an astonishing result''. For me, this is totally over claim without any real application value.
    \item If authors believe that ``This is an astonishing result'', please compare with all the existing Dalle2, stable diffusion methods since they can also do 1 image finetune such as dreambooth type of technology (I know dreambooth is not for 1 image but I mean similar)
    \item In-painting doesn't need any precise mask, simple bursh already working very well. I still believe authors should compare. 
\end{itemize}

\vspace{0.5cm}

\myparagraph{Incorporation of the feedback into the revision.}

\begin{itemize}
    \item \textbf{Reviewer 1.} The initial concerns of reviewer 1 were addressed in the paper revision during the previous submission. After the revision, reviewer 1 recommended acceptance with no further changes. We note that reviewer 1 initially suggested to submit our work to IEEE TIP, which influenced our choice for the resubmission venue. 
    \item \textbf{Reviewer 2.} Our current submission addresses each of the comments of reviewer 2 from the second round. Firstly, the writing of the paper now clearly outlines the difference of our method to image manipulation methods, as well as mentions its advantages over image manipulation methods in some practical scenarios (comments 1-2). Secondly, we adjusted the wording of the claims to avoid concerns on over-claiming (comments 2-3). Thirdly, as suggested by reviewer 2, we added a comparison of our model to recent image manipulation methods, including image in-painting (Sec. \textit{IV-D}, Fig. 11, Table \textit{VII}) (comment 4).
\end{itemize}

\end{comment}
